MiSTiQ: MicroScaling Trellis Quantization for Extreme KV Cache Compression

Modern large language models (LLMs) increasingly support longer contexts and serve more concurrent requests, increasing both sequence lengths and batch sizes. Both trends increase KV-cache size and memory traffic during inference. KV-cache quantization reduces these costs, with recent approaches using codebook-based vector quantization to achieve extremely low bit widths. However, hardware constraints limit codebook size, and most methods reconstruct the cache in higher-precision floating-point formats for attention, limiting the computational benefits of quantization. To address these limitations, we introduce MiSTiQ, a drop-in replacement for codebook-based vector quantizers that combines trellis-coded storage with microscaling (MX) formats for low-precision computation. We combine trellis quantization with beam search to encode the KV cache over large reconstruction spaces without large codebooks. To support MX computation, we derive MX-Hash functions that generate reconstruction values directly in the target MX element format. These functions use the scale-conditioned marginal distribution of block-normalized Gaussian inputs. On Llama3 and Qwen3, MiSTiQ achieves lower WikiText perplexity and higher GSM8K accuracy than the evaluated baselines across several block-scale formats at approximately 1.25 effective bits per element. With NVFP4, it also achieves the highest LongBench average on both models.

==> files/ai_disclosure.tex <==
\section*{AI Usage Disclosure}

We used OpenAI Codex to assist with code development, debugging,
and manuscript preparation. This assistance included generating
and editing portions of the implementation, helping diagnose
and resolve code errors, inspecting the LaTeX project and
accompanying code, refining manuscript language, and checking
the text for clarity and consistency.

The authors retain full responsibility for the correctness,
originality, attribution, and integrity of the submitted work,
including all content produced with AI assistance.

==> files/analysis.tex <==
\section{Block Vector Quantization}
% \subsection{Microscaling Vector Quantization}
Let $\x\in\mathbb{R}^{d}$ denote the full vector to be quantized.
Let $B$ be the MX block size, assume $B$ divides $d$, and define
$N_B=d/B$ contiguous MX blocks $\z_i\in\mathbb{R}^{B}$ by
\[
\x=
\left[
\z_0^{\top},
\ldots,
\z_{N_B-1}^{\top}
\right]^{\top}.
\]
Each MX block receives its own quantized scale. Within each block, let
$m$ be the VQ subvector dimension, assume $m$ divides $B$, and define
$N_V=B/m$ local subvectors. These subvectors are contiguous within a
single $\z_i$ and never cross MX-block boundaries. Let $k\geq 2$ denote the
number of codewords, and let $Q_S$ and $Q_E$ denote the block-scale and
element-format quantizers, respectively. We use one shared
element-format-quantized codebook for all subvectors in all MX blocks:
\[
\overline{\mathcal{C}}
=
\left\{
\bar{\vectorsym{c}}_{\ell}
=
Q_E\brackets{\vectorsym{c}_{\ell}}
\right\}_{\ell=1}^{k},
\]
where $\vectorsym{c}_{\ell}\in\mathbb{R}^{m}$ and $Q_E$ is applied
elementwise; this MX-VQ codebook uses $q=k$ codewords.

For a generic nonzero MX block
$\z\in\mathbb{R}^{B}$,\footnote{All-zero MX blocks are excluded from
this local scale-normalized analysis and require a separate zero-block
convention or implementation path.} let $Q_S$ map positive block maxima to positive
quantized scales and define
\begin{subequations}
\begin{align}
s(\z)
&=
Q_S\brackets{\max_{1\leq r\leq B}\abs{z_r}},
\qquad
\tilde{\z}=\z/s(\z),
\\
\widehat{\z}
&=
s(\z)\QVQ(\tilde{\z},\overline{\mathcal{C}};m,k).
\end{align}
\end{subequations}
Applying this MX-VQ definition independently to each nonzero $\z_i$
with the same shared codebook gives
\[
\widehat{\x}
=
\left[
\widehat{\z}_0^{\top},
\ldots,
\widehat{\z}_{N_B-1}^{\top}
\right]^{\top}.
\]
\subsection{Analysis}
\paragraph{Mean-squared quantization error.}
Let $\x\in\mathbb{R}^{d}$ be a random vector and let
$\widehat{\x}$ denote its quantized reconstruction. We define the
normalized mean-squared error (MSE) as
\begin{equation}
\mseerr
\coloneqq
\frac{1}{d}\,
\mathbb{E}\left[
\norm{\x-\widehat{\x}}_2^2
\right].
\label{eq:mse-definition}
\end{equation}

To expose the contribution of each MX block, partition $\x$ and
$\widehat{\x}$ into corresponding blocks
$\z_i,\widehat{\z}_i\in\mathbb{R}^{B}$. Since the squared Euclidean
norm is additive over disjoint blocks,
\begin{align}
\mseerr
&=
\frac{1}{N_B}
\sum_{i=0}^{N_B-1}
\underbrace{
\frac{1}{B}
\mathbb{E}\left[
\norm{\z_i-\widehat{\z}_i}_2^2
\right]
}_{\blockerr{i}}
\label{eq:mse-block-decomposition}
\end{align}
Here, $\blockerr{i}$ is the per-coordinate MSE of block $i$, and
$\mseerr$ averages these quantities uniformly over the $N_B$
equal-sized blocks.

\begin{proof}
For a nonzero block $\z$, let
$s^*\brackets{\z}=\max_{1\leq r\leq B}\abs{z_r}$ be the reference scale
and let $s\brackets{\z}=Q_S\brackets{s^*\brackets{\z}}$ be its
quantized scale. Define the intermediate reconstructions
$\tilde{\z}=s^*\brackets{\z}\QVQ\brackets{\frac{\z}{s^*\brackets{\z}},\mathcal{C};m,k}$
and
$\overline{\z}=s\brackets{\z}\QVQ\brackets{\frac{\z}{s\brackets{\z}},\mathcal{C};m,k}$,
and let
$\widehat{\z}=s\brackets{\z}\QVQ\brackets{\frac{\z}{s\brackets{\z}},\overline{\mathcal{C}};m,k}$
be the final reconstruction using the element-format-quantized codebook.
\begin{equation}
    \norm{\z-\widehat{\z}}_2\leq \norm{\z-\tilde{\z}}_2+\norm{\tilde{\z}-\overline{\z}}_2+\norm{\overline{\z}-\widehat{\z}}_2
\end{equation}
For the ideal codebook $\mathcal C$ supplied by
\cref{lem:vq-worst-case-upper-bound}, the first term satisfies
\begin{equation}
\norm{\z-\tilde{\z}}_2
=
s^*\brackets{\z}
\norm{
\frac{\z}{s^*\brackets{\z}}
-
\QVQ\brackets{\frac{\z}{s^*\brackets{\z}},\mathcal{C};m,k}
}_2
\leq
\frac{s^*\brackets{\z}\sqrt{B}}{\left\lfloor k^{1/m}\right\rfloor},
\label{eq:ideal-codebook-error-bound}
\end{equation}
where the inequality uses \cref{lem:vq-worst-case-upper-bound} with
$d=B$ and $A=1$, since $\z/s^*\brackets{\z}\in[-1,1]^B$.
\begin{align}
    \norm{\tilde{\z}-\overline{\z}}_2=s^*\brackets{\z} \norm{\QVQ\brackets{\frac{\z}{s^*\brackets{\z}},\mathcal{C};m,k}-\frac{s\brackets{\z}}{s^*\brackets{\z}}\QVQ\brackets{\frac{\z}{s\brackets{\z}},\mathcal{C};m,k}}
\end{align}
\end{proof}
% Thus, the global error is the sum of the normalized contributions from
% the individual MX blocks. Equivalently, if the per-block MSE is defined
% as
% \begin{equation}
% \blockmse{i}
% \coloneqq
% \frac{1}{B}
% \mathbb{E}\left[
% \norm{\z_i-\widehat{\z}_i}_2^2
% \right],
% \end{equation}
% then $d=N_BB$ gives
% \begin{equation}
% \mseerr
% =
% \frac{1}{N_B}
% \sum_{i=0}^{N_B-1}\blockmse{i}.
% \label{eq:mse-average-blocks}
% \end{equation}


==> includes/results/ablation_ppl_per_bit_mxblock.tex <==
% % Requires: \usepackage{caption}
% \begin{table}[t]
% \centering
% \captionsetup{justification=centering,singlelinecheck=false}
% \caption{MX block-size ablation for Llama-3.1-8B-Instruct.
% QTIP MX-Hash with the NSN backbone, UE5M3 joint scales,
% E2M1, $V4$, $T1024$, uniform K/V payloads of 1 bit,
% and beam 128. The bit--PPL product is effective bits
% $\times$ perplexity; lower is better. Bold marks each column's minimum.}
% \label{tab:mx-blocksize-nsn}
% \begingroup
% \footnotesize
% \setlength{\tabcolsep}{6pt}
% \setlength{\arrayrulewidth}{0.3pt}
% \renewcommand{\arraystretch}{1.35}
% \begin{tabular}{@{}c|ccc@{}}
% \hline
% Block size $G$ &
% \shortstack{Effective\\Bit} &
% Perplexity $\downarrow$ &
% \shortstack{Bit--PPL\\product $\downarrow$} \\
% \hline
% 32   & 1.4961 & \textbf{10.373} & 15.520 \\
% 64   & 1.3711 & 10.607 & 14.543 \\
% 128  & 1.3086 & 10.699 & 14.001 \\
% 256  & 1.2773 & 10.882 & 13.900 \\
% 512  & 1.2617 & 10.818 & 13.650 \\
% 1024 & 1.2539 & 10.874 & \textbf{13.635} \\
% \hline
% \end{tabular}
% \endgroup
% \end{table}

% In the preamble:

% Put the SVG in figures/:
\begin{figure}[t]
    \centering
    \includesvg[width=0.7\linewidth]{figures/results_figures/nsn_mx_blocksize_clean.svg}
    \caption{Effect of MX block size on effective bits and perplexity.}
    \label{fig:mx-blocksize}
\end{figure}

==> includes/results/ablation_vector_length_payload.tex <==
% % Requires: \usepackage{caption}
% \begin{table*}[t]
% \centering
% \captionsetup{justification=centering,singlelinecheck=false}
% \caption{Perplexity ($\downarrow$) for the payload-flexibility ablation
% of QTIP MX-Hash with the NSN backbone and joint UE5M3 scales.
% All variants use $G128$, $T1024$, beam 128, and 1.3086 effective
% bits per element. K/V payloads are bits per element.
% Bold marks the best available result; --- denotes unavailable results.}
% \label{tab:payload-flexibility}
% \begingroup
% \footnotesize
% \setlength{\tabcolsep}{6pt}
% \setlength{\arrayrulewidth}{0.3pt}
% \renewcommand{\arraystretch}{1.35}
% \begin{tabular}{@{}ccc|cc@{}}
% \hline
% \shortstack{Vector\\length} &
% \shortstack{K\\payload} &
% \shortstack{V\\payload} &
% Llama-3.1-8B-Instruct &
% Qwen3-8B \\
% \hline
% V2 & 1.000 & 1.000 & 10.929 & 14.951 \\
% V4 & 1.000 & 1.000 & 10.699 & 14.942 \\
% V4 & 1.250 & 0.750 & \textbf{10.698} & \textbf{13.089} \\
% V8 & 1.000 & 1.000 & --- & --- \\
% V8 & 1.125 & 0.875 & --- & --- \\
% \hline
% \end{tabular}
% \endgroup
% \end{table*}

% Requires: \usepackage{caption}
\begin{table*}[t]
\centering
\captionsetup{justification=centering,singlelinecheck=false}
\caption{Perplexity ($\downarrow$) on Llama-3.1-8B-Instruct for the
payload-flexibility ablation of QTIP MX-Hash with the NSN backbone
and joint UE5M3 scales. All variants use one H100 GPU, $G128$,
$T1024$, beam 128, and 1.3086 effective bits per element.
K/V payloads are bits per element. Bold marks the best result.
}
\todo[inline]{Consider moving to appendix and replacing with V4 V8 per payload figure}
\label{tab:payload-flexibility}
\begingroup
\footnotesize
\setlength{\tabcolsep}{6pt}
\setlength{\arrayrulewidth}{0.3pt}
\renewcommand{\arraystretch}{1.35}
\begin{tabular}{@{}ccc|c@{}}
\hline
\shortstack{Vector\\length} &
\shortstack{K\\payload} &
\shortstack{V\\payload} &
Llama-3.1-8B-Instruct \\
\hline
V2 & 1.000 & 1.000 & 10.929 \\
V4 & 1.000 & 1.000 & 10.699 \\
V4 & 1.250 & 0.750 & 10.698 \\
V8 & 1.125 & 0.875 & \textbf{10.531} \\
\hline
\end{tabular}
\endgroup
\end{table*}

==> includes/results/below_1bit_ppl.tex <==
% Requires: \usepackage{multirow,graphicx} and \usepackage[table]{xcolor}
% Generated by build_table.py; best cell fill 9DC3E6; black text.
% Source: experiments/00-official/v3/results.xlsx; SHA256 99c4bb04f8c77a6d87baf4746bf35250d7df9f04cc35469a810f06fcf68716f7
% Source: experiments/00-official/v4/results_v4.xlsx; SHA256 9fd044211551b2901e38fc8ff876f7190caf2a1a1bd93117c0de1d37d46579c5
\begin{table*}[!h]
\centering
\color{black}
\caption{Below-1-bit MX KV-cache quantization perplexity, with a 1-bit VecInfer reference. Effective Bit denotes mean effective bits per element using dynamic storage accounting. Within each block-scale format and model, dark blue cells mark the lowest perplexity and light blue cells mark the second-lowest perplexity among the displayed quantized methods, excluding BF16; ties share a color.}
\label{tab:below-one-bit-ppl}
\begingroup
\footnotesize
\setlength{\tabcolsep}{3pt}
\setlength{\arrayrulewidth}{0.3pt}
\renewcommand{\arraystretch}{1.35}
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{@{}ccc|c|c@{}}
\hline
\shortstack{Block-scale\\format} & Variant & \shortstack{Effective\\Bit} & \textbf{Llama-3.1-8B-Instruct} & \textbf{Qwen3-8B} \\
\hline
--- & BF16 & 16.00 & 7.170 & 9.750 \\
\hline
\multirow{4}{*}{UE8M0} & VecInfer & 1.00 & 693.850 & 409.782 \\
 & NSN & 0.99 & \cellcolor[HTML]{DDEBF7}\color{black} 52.257 & 80.740 \\
 & QTIP MX-Hash & 0.99 & \cellcolor[HTML]{9DC3E6}\color{black} 38.315 & \cellcolor[HTML]{9DC3E6}\color{black} 57.616 \\
 & QTIP MX-Hash & 0.93 & 57.510 & \cellcolor[HTML]{DDEBF7}\color{black} 79.069 \\
\hline
\multirow{4}{*}{UE5M3} & VecInfer & 1.00 & 694.108 & 324.561 \\
 & NSN & 0.99 & 54.845 & 87.735 \\
 & QTIP MX-Hash joint & 0.99 & \cellcolor[HTML]{9DC3E6}\color{black} 32.136 & \cellcolor[HTML]{9DC3E6}\color{black} 42.248 \\
 & QTIP MX-Hash joint & 0.93 & \cellcolor[HTML]{DDEBF7}\color{black} 45.496 & \cellcolor[HTML]{DDEBF7}\color{black} 59.141 \\
\hline
\end{tabular}
}
\endgroup
\end{table*}

==> permutation_ilp_formulation.tex <==
% Requires \usepackage{amsmath,amssymb}

\section{Permutation ILP}
Consider one KV head with head dimension $D$ and quantization block
size $B$, where each quantization block contains $B$ channels that
share one quantization scale. We assume that $B$ is even and divides
$D$.

Let $x_{tc}$ denote channel $c$ of the key or value vector captured at
token position $t$. The batch and token dimensions of the calibration
data are flattened to form
\[
X\in\mathbb{R}^{R\times D},
\]
where each of the $R$ rows is one captured token's $D$-dimensional
key or value vector.

Under the default RoPE-pair-preserving policy, the solver permutes
adjacent channel pairs rather than individual channels. Each pair
$(2j,2j+1)$ is treated as one indivisible permutation unit: its two
channels remain together, while the pair may be assigned to any
quantization block.

Consequently, the number of permutation units is $U=\frac{D}{2}$,
the number of units in each quantization block is
$K=\frac{B}{2}$,
and the number of quantization blocks is
$N_B=\frac{U}{K}=\frac{D}{B}$.
Define
\[
\mathcal T=\{0,\ldots,R-1\},\qquad
\mathcal J=\{0,\ldots,U-1\},\qquad
\mathcal B=\{0,\ldots,N_B-1\}.
\]
Here, $\mathcal T$ is the set of calibration-row indices,
$\mathcal J$ is the set of permutation-unit indices, and
$\mathcal B$ is the set of quantization-block indices.
For calibration value $x_{tc}$, define the normalized magnitude of
unit $j$ in row $t$ as
\[
a_{tj}
=
\frac{\max\{|x_{t,2j}|,\ |x_{t,2j+1}|\}}{s},
\qquad
s=
\max\left\{
10^{-12},
\max_{t\in\mathcal T,\;j\in\mathcal J}
\max\{|x_{t,2j}|,\ |x_{t,2j+1}|\}
\right\}.
\]
Let $z_{jb}\in\{0,1\}$ indicate whether unit $j$ is assigned to block
$b$, and let $y_{tb}\in[0,1]$ represent the maximum magnitude assigned
to block $b$ in row $t$. The optimization problem is
\[
\begin{aligned}
\min_{z,y}\quad
    & \sum_{t\in\mathcal T}\sum_{b\in\mathcal B} y_{tb}
\\
\text{s.t.}\quad
    & \sum_{b\in\mathcal B} z_{jb}=1,
    && \forall j\in\mathcal J,
\\
    & \sum_{j\in\mathcal J} z_{jb}=K,
    && \forall b\in\mathcal B,
\\
    & y_{tb}\ge a_{tj}z_{jb},
    && \forall t\in\mathcal T,\ b\in\mathcal B,\ j\in\mathcal J,
\\
    & z_{jb}\in\{0,1\},
    && \forall j\in\mathcal J,\ b\in\mathcal B,
\\
    & 0\le y_{tb}\le1,
    && \forall t\in\mathcal T,\ b\in\mathcal B.
\end{aligned}
\]
At the optimum,
\[
y_{tb}=\max_{j:z_{jb}=1}a_{tj},
\]
so the objective minimizes the sum, over calibration rows and
quantization blocks, of the maximum magnitude within each block.


==> section_files/efficient_implementation.tex <==
\section{Efficient Implementation}
\label{sec:efficient-implementation}

We propose an efficient implementation for \MN{} aimed at minimizing incremental inference latency. We consider encoding and decoding separately. For encoding, GPU support for concurrent kernel execution motivates overlapping beam search with independent GEMM computation.\footnote{NVIDIA, \emph{CUDA C++ Best Practices Guide}, Concurrent Kernel Execution: \url{https://docs.nvidia.com/cuda/cuda-c-best-practices-guide/index.html\#concurrent-kernel-execution}.} When the execution schedule first requires the encoded KV entries for the next generated token, this overlap could hide encoding latency, provided that encoding completes before their use and resource contention does not extend execution. For decoding, building on hardware-efficient trellis decoding \citep{tseng2025qtip}, we propose a lookup-table implementation of the MX-Gaussian hash that replaces inverse-CDF evaluation with table accesses, comparisons, and elementary arithmetic on the table-covered range.

\paragraph{Encoding.}
Encoding can begin as soon as the required KV entries are available, and it can proceed concurrently with later GEMMs and the attention dot product, which use the uncompressed output during prefill or when decoding a token. Assume that between generating a layer’s KV-cache token and the next attention step, there are several large GEMMs and an attention dot product; this can allow the encoding latency to be hidden within that computation window.

\paragraph{Decoding.} 
Specifically, we factor the scale-conditioned inverse CDF using the coefficients in \cref{eq:lut-coefficients}. For every supported positive finite scale $s$, we precompute the slopes $\lutslopes_0(s),\lutslopes_1(s)$, offset $\lutoffset(s)$, branch threshold $p^\star(s)$, and prefactor $\sqrt2/s$. Given the midpoint probability $p_\ell$ and sign bit $\mxsignbit_\ell$ from \cref{eq:mx-hash-sign-rank,eq:mx-hash-interior-probability}, the inverse-error-function argument is
\begin{equation}
\lutargument_\ell=
\begin{cases}
\lutslopes_0(s)p_\ell, & p_\ell\le p^\star(s),\\
\lutslopes_1(s)p_\ell+\lutoffset(s), & \text{otherwise}.
\end{cases}
\label{eq:efficient-main-affine}
\end{equation}
This leaves a shared scalar inverse error function to approximate. We propose 256 uniformly spaced finite knots
$0=\lutknots_0<\cdots<\lutknots_{255}<1$ and store
$\lutvalues_j=\stdierf(\lutknots_j)$.
For $\lutknots_j\le\lutargument_\ell\le\lutknots_{j+1}$, with $0\le j\le254$, evaluate
\begin{equation}
\begin{aligned}
\lutfunction(\lutargument_\ell)
&=\lutvalues_j+
 \frac{\lutargument_\ell-\lutknots_j}
      {\lutknots_{j+1}-\lutknots_j}
 (\lutvalues_{j+1}-\lutvalues_j),\\
\widehat h_{\hashparams,\ell}(u;s)
&=Q_E\!\left(
(-1)^{\mxsignbit_\ell}\frac{\sqrt2}{s}
\lutfunction(\lutargument_\ell)\right).
\end{aligned}
\label{eq:efficient-main-interpolation}
\end{equation}
% Uniform spacing permits arithmetic interval selection and one shared precomputed reciprocal spacing, so interpolation requires no runtime division. The endpoint uses the final interval. The scale prefactor is also precomputed. Together with the existing integer mixer, the covered path uses bit operations, integer and floating-point arithmetic, comparisons, table accesses, sign restoration, and element quantization. The output remains a normalized element; block reconstruction additionally applies the represented block scale.

% Five FP32 coefficients for each of 256 scale slots require 5\,KiB, while the two 256-entry FP32 knot and value arrays require 2\,KiB. The base tables therefore occupy 7\,KiB, plus one FP32 reciprocal spacing and implementation alignment. No interval-slope array is needed. Any higher-precision coefficient storage or fallback-specific data is additional to this base footprint.

% The singular endpoint $\stdierf(1)$ is never tabulated. Arguments outside the finite table range use the full scale-conditioned inverse CDF, with its cost included in any performance assessment. Probability and coefficient evaluation must preserve interior arguments: FP32 alone cannot distinguish all 31-bit midpoint ranks and may round the largest probabilities to one. Stable evaluation, using higher precision where required, is therefore part of the implementation. Table spacing, arithmetic precision, and tail frequency must be validated for the supported scales; the approximation need not preserve every element-rounding decision. This is an implementation proposal, not a measured decoder-speedup or negligible-latency result.


==> section_files/hash_search_experiment_details.tex <==
\section{Hash-search experiment details}
\label{app:hash-search-experiment-details}

This appendix specifies the two synthetic comparisons in
Figure~\ref{fig:hash-search-comparison}. Panel (a) compares four configured
hash methods with fixed initial scales. Panel (b) holds the MX-Gaussian
provider and beam width fixed and compares two output-scale strategies.
The Gaussian mixer was selected in a historical training campaign; the
three fixed baselines receive no comparable selection budget.

\paragraph{Data and error measure.}
Each of seeds 42001--42005 supplies eight held-out rows of 128 independent
standard normal coordinates. NumPy's PCG64 generator draws
\texttt{standard\_normal} in float64 and casts once to float32.
Panel (a) uses these exact 40 rows. For panel (b), each saved row is extended
to length 2048 with an independent Gaussian tail. The tail generator uses
\texttt{SeedSequence([20261004, seed, row])}, with zero-based row indices,
and again casts float64 normal draws once to float32. Every tested length
uses the corresponding prefix of that same saved row; lengths 32 and 64
therefore need no new input randomness. Original 128-coordinate prefixes
remain unchanged, and both strategies receive identical inputs at each
length. The tested lengths are 32, 64, 128, 256, 1024 and 2048.

Inputs are not clipped. Initial-scale normalization is internal to search.
Every plotted point averages 40 original-domain per-row MSEs, equivalently
pooling all coordinates because rows at a point have equal length.
Independent audit subtracts the final float32 reconstruction from the
original float32 input in float64. The plotted MSE uses the final represented
UE5M3 scale, including rounding after continuous fitting; it is not the
solver's unrounded fitted-scale diagnostic or energy-normalized error.
The original program-selection cohorts use seed 42000 for a one-row pilot
and seed 43000 for eight training rows.

\paragraph{Geometry and fixed initial scales.}
The element format is FP4 E2M1 with finite magnitudes
$\{0,0.5,1,1.5,2,3,4,6\}$, nearest-even rounding and signed zero.
Every 32-coordinate block receives the nearest positive UE5M3 scale to its
absolute maximum divided by six, with lower-scale midpoint ties; an all-zero
block uses scale one. Legal positive scale codes are 1--255.
Fixed-scale search retains this initial scale throughout each block and
searches only the trellis path. It does not enumerate scale candidates.
Targets are divided by the initial scale, and initial-scale error weights
restore the original-domain squared-error objective.

The state width is $L=16$ (65536 states), with 8 start bits (256 allowed
starts). There are $V=4$ emissions per transition at rate two bits per scalar:
eight transition bits give 256 successors per state. Trellis state and cost
continue across MX blocks. A length-128 row has 32 transitions and four
blocks; lengths 32 and 64 have eight and sixteen transitions respectively.
Panel (a) varies beam width over 32, 64, 128, 256, 512, 1024, 2048 and 4096.
Both strategies in panel (b) use width 1024. Beam pruning uses stable cost
order, parent-major then ascending transition symbol, without epsilon ties.

\paragraph{Continuous joint scale fitting.}
The continuous solver retains the existing sufficient-statistic objective.
Within each block, it accumulates squared emissions and normalized
target--emission products for each candidate path. In an unfinished block,
the fitted amplitude ratio has a unit-weight regularizer toward one
(\texttt{alpha=1}). At the block boundary, the solver removes this regularizer
and commits the positive least-squares amplitude for each retained path.
After recovering the winning path, it rounds the fitted absolute scales to
nearest positive UE5M3, with lower midpoint ties. Prefix pruning uses
continuous fitted amplitudes; final rounded-scale MSE is recomputed
separately rather than assumed to equal the internal search cost.

For both Gaussian strategies, let $\mxguidescale_b$ denote the initial
represented scale that conditions the emission guide, and let
$\mxoutscale_b$ denote the final represented reconstruction scale.
The guide scale remains fixed throughout the block. In fixed-scale search,
$\mxoutscale_b=\mxguidescale_b$. Continuous fitting changes only the output amplitude. With quantized
guide emissions $\widehat{\x}_b$, reconstruction is
$\widehat{\y}_b=\mxoutscale_b\widehat{\x}_b$, while the emissions are
evaluated using $\mxguidescale_b$. The final represented amplitude replaces
the initial reconstruction multiplier; the two amplitudes are not multiplied
together. Initial conditioning codes and final output codes are saved
separately, and replay uses the former to emit values and the latter to
reconstruct them.

\paragraph{Conditional Gaussian guide.}
MX-Gaussian denotes the conditional CDF hash of
Section~\ref{sec:mx-hash}, using the scale-cell guide in
Theorem~\ref{thm:mx-gaussian-conditional}. The theorem's interpretation remains
conditional on its stated maximum-based scale event. A fitted output scale
does not redefine the initial-code conditioning event.

The hash uses the existing unsigned 32-bit LCG and XOR--multiply program,
in the order LCG, mixer, sign/rank. The high bit selects the sign;
the remaining 31 bits give midpoint probabilities $(U_\ell+1/2)/2^{31}$.
The conditional inverse magnitude guide is followed by native FP4 rounding.
These are deterministic maps of states and output coordinates, not claims of independent
Gaussian outputs. Numerical cutpoints use adaptive high-precision convergence
checks with explicit limits; those checks are not formal interval proofs.
Audit reconstructs emissions from independent inverse references rather than
from the prepared boundary table.

\paragraph{Fixed baselines.}
For 1MAD, generating each output coordinate applies its fixed unsigned 32-bit LCG, sums the four bytes,
subtracts 510 and divides in float32 by 147.8. For 3INST, the LCG word for each output coordinate
is masked by hexadecimal \texttt{8fff8fff}, then XORed with
\texttt{3b603b60}. Its two halves are reinterpreted as FP16; their sum is
rounded to FP16, converted to float32 and divided by float32 1.24.
The four LCG pairs for 1MAD are the shared Gaussian pairs in
Table~\ref{tab:hash-search-programs}; those for 3INST, in output coordinate order, are
$(89226354,64248484)$, $(4035414189,2926533967)$,
$(3229444775,3165951693)$ and $(240516867,909804477)$.

For each of these two baselines, the alignment factor is eight divided by the
maximum absolute value over its complete $65536\times4$ regular table.
The applied factor and multiplication are float32, followed by nearest-even
FP4 rounding \emph{inside} search. Thus search scores the original target
against the represented scale times this rounded, aligned emission.
These baseline emission tables use no target-dependent fitting. Full regular, scaled and rounded table
digests and the requested/applied factors are retained in the row metadata.

The Heuristic FP label uses the same original 3INST arithmetic with the
fixed block-32 factor $\fpclipfactor=1/\sqrt{2\ln(32/\pi)}$ from
Section~\ref{sec:mx-hash}. Its operation order is float32 multiplication by
$\fpclipfactor$, clipping to $[-1,1]$, float32 multiplication by six, and nearest-even
FP4 rounding inside search. It receives neither the full-domain eight/maximum
alignment nor mixer training. This declared in-search adaptation does not
claim equivalence to an upstream postdecode quantizer's tie or zero behavior.
The experiment does not sweep or validate the choice of $\fpclipfactor$.

\paragraph{Historical program pool and selection.}
The Gaussian mixer program is reused without retraining from the original
exact-search selection campaign. PCG64 seed 43001 supplied ten distinct
random programs with four output coordinates. No initial program was forced into the pool.
For each proposal and output coordinate, the generator first draws three integer shifts
uniformly from 1 through 31, then two integers uniformly from 0 through
$2^{31}-1$, mapping each to an odd multiplier by doubling and adding one.
LCG pairs remain fixed. Complete RNG states, proposal indices and duplicate
redraws are saved. This pool required ten proposals and no duplicate redraw;
a 1000-proposal cap would fail rather than accept a partial pool.

Historical training evaluated each program by exact search on eight rows
at nominal candidate-slot counts $K=2,3,5,9$ under
\texttt{canonical\_offsets\_v2}. Their code offsets were $(0,1)$,
$(-1,0,1)$, $(-3,-2,-1,0,1)$ and $(-7,-6,-5,-4,-3,-2,-1,0,1)$,
respectively, relative to the initial code, with legal-range clipping,
stable deduplication and masked padding. Thus each block has at most $K$
unique represented candidates after clipping and deduplication. These candidate sets describe
historical mixer selection only; neither current panel searches these sets.
Selection minimized the equal-weight mean original-domain MSE over the
four candidate counts and eight rows, breaking ties by earliest zero-based
pool index. The conditional Gaussian winner is index 8, with historical
training mean 0.063040330. Its exact output coordinate parameters are frozen across every
current beam width, length and scale strategy. No held-out row enters
selection. Table~\ref{tab:hash-search-programs} records the selected program;
the operations follow
Equations~\ref{eq:mx-hash-lcg}--\ref{eq:mx-hash-mixer}.

\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{crr}
\toprule Output coordinate & LCG multiplier & LCG addend\\\midrule
1 & 34038481 & 76625530\\
2 & 1207148207 & 245029595\\
3 & 2495950493 & 2966120613\\
4 & 4051977331 & 4250177552\\
\bottomrule\end{tabular}
\par\medskip
\begin{tabular}{clrrr}
\toprule Family & Output coordinate & Shifts $(r_1,r_2,r_3)$ & $m_1$ & $m_2$\\\midrule
Conditional & 1 & (1,10,4) & 706914347 & 3570239205\\
Conditional & 2 & (14,6,26) & 2159520081 & 4238934085\\
Conditional & 3 & (22,2,28) & 3180538953 & 1603995129\\
Conditional & 4 & (28,14,5) & 3900032603 & 1727582033\\
\bottomrule\end{tabular}
\caption{Full selected output coordinate parameters. The Gaussian hash and 1MAD use the shared LCG pairs above. Mixer field meanings follow the existing hash equations.}
\label{tab:hash-search-programs}
\end{table}

\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{rrrrr}
\toprule Width & MX-Gaussian & 1MAD & 3INST & Heuristic FP\\\midrule
32 & 0.072729554 & 0.078570861 & 0.075074020 & 0.074770146\\
64 & 0.070854322 & 0.075333632 & 0.072912563 & 0.072636581\\
128 & 0.069618485 & 0.074172798 & 0.070643667 & 0.071371940\\
256 & 0.068666903 & 0.073726164 & 0.070070612 & 0.070640645\\
512 & 0.068252374 & 0.073453713 & 0.069971118 & 0.070402059\\
1024 & 0.067997618 & 0.073090538 & 0.069715552 & 0.070270028\\
2048 & 0.067655660 & 0.072979156 & 0.069655587 & 0.070072866\\
4096 & 0.067655660 & 0.072786674 & 0.069594781 & 0.069893559\\
\bottomrule\end{tabular}
\caption{Final MSE for fixed initial UE5M3 scales at trellis length 128. MX-Gaussian uses frozen winner 8; Heuristic FP is the fixed-factor 3INST adaptation.}
\label{tab:hash-search-width}
\end{table}

\begin{table}[t]
\centering\small
\begin{tabular}{rrr}
\toprule Length & Fixed initial scale & Continuous joint search\\\midrule
32 & 0.053171649 & 0.048553808\\
64 & 0.063463152 & 0.058945954\\
128 & 0.067997618 & 0.063039714\\
256 & 0.068569715 & 0.063827187\\
1024 & 0.069540802 & 0.064930463\\
2048 & 0.069648399 & 0.065135756\\
\bottomrule\end{tabular}
\caption{Final MSE for the two MX-Gaussian scale strategies at beam width 1024. Both condition emissions on initial codes; continuous output amplitudes are rounded to UE5M3 before measuring error.}
\label{tab:hash-search-length}
\end{table}

\paragraph{Independent checks and scope.}
Saved starts and symbols independently rebuild trellis states. Gaussian
replay uses the initial conditioning codes and independent inverse
references. Static replay starts from original arithmetic; heuristic replay
independently reproduces its integer, FP16, float32 and nearest-even
operations. Final output codes independently recover UE5M3 amplitudes and
physical reconstructions. Audit requires bitwise reconstruction identity,
including signed zero, checks continuous fitted scales against independent
least-squares statistics within native float32 tolerance, and checks final
UE5M3 rounding independently.

The original fixed/continuous campaign replayed all 1960 rows and 13 pilot
controls. The updated figures retain 1560 of those solves and add 160 new
length-32/64 solves, with four separate pilot controls. All 1720 unique
retained/new rows passed independent replay. The beam and length panels
contain 1280 and 480 row results respectively, sharing 40 fixed Gaussian
length-128/width-1024 results.

Tables~\ref{tab:hash-search-width} and~\ref{tab:hash-search-length}
reproduce the plotted means, rounded to nine decimal places;
the coordinate CSVs retain full numerical precision, row standard
deviations and standard errors. Continuous fitting gives lower mean final
MSE than fixed initial scales at each tested length in this cohort.
These observations concern the configured methods, selected Gaussian
program and forty synthetic rows. They do not establish universal
dominance, monotone finite-beam performance, or a guaranteed improvement
from fitting followed by scale rounding.

\paragraph{Execution and resource reporting.}
New searches run sequentially on explicit native MPS outside the sandbox
with \texttt{PYTORCH\_ENABLE\_MPS\_FALLBACK=0}; unavailable MPS or fallback
is a failure. CPU inverse replay is an audit oracle rather than a substitute
search backend. The recorded environment is macOS 26.6.2 arm64, Python
3.13.9, PyTorch 2.14.0, NumPy 2.5.3, SciPy 1.18.0 and mpmath 1.3.0.
Row telemetry records process RSS high-water usage and native MPS allocator
and driver memory. The observed RSS policy is 2 GiB, and observed allocator
growth above each row's baseline is limited to 512 MiB. Memory samples have
a 100-millisecond period and boundary samples; they do not prove exact
transient peaks. Synchronized setup, search and replay timings are retained
separately as diagnostics, without speedup claims.

\paragraph{Artifacts and reproduction.}
{\small\raggedright
The historical selection root is
\path{experiments/joint_scale_comparison/runs/20260925_v2_best10_ue5m3},
with manifest
\path{f62f5ee5e1e062e5b08567f86c7e5585d5e31c0f027a1a274191ac09ee2e42a9}.
The fixed/continuous parent root is
\path{experiments/fixed_scale_comparison/runs/20261004_initial_ue5m3_r3},
with manifest
\path{ed421ff900d2215fad779d7d90dc486cd285543e2d2f737c625139b6e27821f4}.
The updated figure root is
\path{experiments/fixed_scale_comparison/runs/20261004_initial_ue5m3_update},
with manifest
\path{434c708bbb3ad1ade9d922a248e9c1835bc19644d34b7c54e2b8a9b175048ac7}.
It contains \path{beam_coordinates.csv}, \path{length_coordinates.csv},
\path{manifest.json}, \path{audit.json}, \path{report.json}, per-row
archives and completion records, and
\path{rendering_provenance.json}. Its immutable manifest authenticates
original artifacts, saved inputs, frozen programs, current numerical
sources, artifact-side scripts and runtime. Historical source identities
remain distinct from current execution identity. The recorded
\texttt{lcg\_source} namespace relocation changes metadata only; both
original and resolved program hashes are retained, with exact constants,
mixers, rank and ordering semantics checked.
\par}

{\raggedright
To reproduce the fixed/continuous parent, obtain the source bytes and
environment recorded in its manifest. Hashes do not provide recoverable
source archives. Run outside the sandbox, set
\texttt{PYTORCH\_ENABLE\_MPS\_FALLBACK=0} before Python starts, and invoke
\path{mx_qtip_quantization.analyze_experiment.fixed_scale_comparison}
with \texttt{python -m}. Choose one fresh \texttt{--output} root and use
stages \texttt{check}, \texttt{pilot}, \texttt{run}, \texttt{audit} and
\texttt{plot}, with \texttt{--parent} pointing to the pinned historical
selection campaign. The artifact-side update script \path{run_update.py}
uses the same ordered stages and the authenticated saved parent inputs.
Its output root is its own directory, and it adds only the length-32/64
solves before replaying the retained results and plotting the updated views.
Atomic row checkpoints and a single-writer lock permit exact resume.
Identity drift, corrupt or orphaned archives fail rather than substituting
a new objective. Later source changes require a new run root rather than
rewriting historical manifests.
\par}


==> section_files/hash_search_figure.tex <==
\begin{figure*}[t]
  \centering
  \captionsetup{skip=3pt}
  \captionsetup[subfigure]{skip=1pt}
  \begin{subfigure}[t]{.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/hash_search/a_fixed_scale_beam.pdf}
    \caption{Fixed initial scale: beam width.}
    \label{fig:hash-search-beam}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/hash_search/b_gaussian_scale_length.pdf}
    \caption{MX-Gaussian: trellis length.}
    \label{fig:hash-search-length}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{.32\textwidth}
    \centering
    \includesvg[inkscapelatex=false,inkscapepath=.build/svg-inkscape/,width=\linewidth]{figures/beam_vs_viterbi}
    \caption{Beam search versus Viterbi.}
    \label{fig:beam_vs_viterbi}
  \end{subfigure}

  \caption{(a,b) Final reconstruction MSE with FP4 E2M1 elements, positive UE5M3
  scales and 32-coordinate MX blocks, averaged over 40 paired synthetic rows
  per point. (a) Four hash methods use fixed initial scales at trellis length
  128 and beam widths 32--4096. (b) At beam width 1024, MX-Gaussian compares
  fixed initial scales with continuous joint scale fitting followed by UE5M3
  rounding, at lengths 32, 64, 128, 256, 1024 and 2048. In (a,b), Gaussian conditioning
  uses the initial guide scale $\mxguidescale_b$ in both searches; the final
  represented output scale $\mxoutscale_b$ multiplies the emission once
  (the two scales coincide in fixed-scale search). Details are in
  Appendix~\ref{app:hash-search-experiment-details}.
  (c) Gaussian inputs on a shared trellis with 256 starts; beam search retains
  duplicate-state paths. Mean \(\pm 1\) sample SD over ten seeds.}
  \label{fig:hash-search-comparison}
\end{figure*}


==> section_files/mixing_parameter.tex <==

\section{Mixing Parameter}
\label{app:mixing-parameter}
\todo[inline]{Implementation deatiles}
We select the post-LCG mixing parameters by reproducible offline random search, keeping the original LCG coefficients \(A_\ell,C_\ell\) fixed. Each candidate specifies all \(V\) output coordinates: draw three shifts per output coordinate uniformly from \(\{1,\ldots,31\}\), and two odd unsigned 32-bit multipliers as \(2q+1\), with \(q\) uniform on \(\{0,\ldots,2^{31}-1\}\). Every candidate quantizes the same fixed Gaussian training vectors. We select the parameters with the smallest mean original-domain reconstruction MSE:

\[
J(\Omega)=\frac{1}{NT}\sum_{n=1}^{N}
\left\|\mathbf y^{(n)}-\widehat{\mathbf y}^{(n)}(\Omega)\right\|_2^2.
\]

Here, \(N\) is the number of fixed Gaussian training vectors, each containing \(T\) coordinates, and \(\Omega\) collects the mixer parameters of all \(V\) output coordinates. The original-domain reconstruction \(\widehat{\mathbf y}^{(n)}(\Omega)\) includes represented-scale and element rounding under fixed quantizer search settings. We minimize \(J\) over the candidate parameter sets, break ties by the earliest candidate index, and freeze the selected parameters for evaluation and decoding.


==> section_files/notation_table.tex <==
\clearpage
\section{Notation}
\label{app:notation}

Symbols used in the compiled paper are grouped within one table. Reused
letters are distinguished by their arguments, indices, and domains.
The block-aligned MX construction additionally assumes $V$ divides $\dmx$;
the generic QTIP background requires only $V\mid T$.

\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.16}
\begin{longtable}{@{}p{0.25\linewidth}p{0.53\linewidth}p{0.17\linewidth}@{}}
\caption{Notation used in the compiled paper.}\label{tab:notation}\\
\toprule Symbol & Meaning, domain, and constraints & Definition \\
\midrule
\endfirsthead
\toprule Symbol & Meaning, domain, and constraints & Definition \\
\midrule
\endhead
\midrule
\multicolumn{3}{r}{\small Continued on the next page}\\
\endfoot
\bottomrule
\endlastfoot
\multicolumn{3}{@{}l}{\textbf{Geometry and microscaling}}\\*
$d,\ T$ & Scalar target length $d=T\in\mathbb N$, $\dmx\mid d$; distinct from trellis outdegree $d$. & \cref{sec:mx-background,sec:mx-methods} \\
$\dmx,\ \mxnumblocks$ & MX block size $\dmx=32$; number of blocks $\mxnumblocks=d/\dmx$. & \cref{sec:mx-background} \\
$b,\ \mxindexset_b$ & Block index $0\le b<\mxnumblocks$; $\mxindexset_b=\{b\dmx,\ldots,(b+1)\dmx-1\}$. & \cref{sec:mx-background} \\
$\y,\ \y_b$ & Target vector in $\mathbb R^d$ and its block in $\mathbb R^{\dmx}$. & \cref{sec:mx-background} \\
$\x_b,\ \widehat{\x}_b$ & Normalized target $\x_b=\y_b/s_b$ and element-grid reconstruction. & \cref{sec:mx-methods} \\
$s_b,\ \widehat{\y}_b$ & Represented block scale; $\widehat{\y}_b=s_b\widehat{\x}_b$. Normalization requires $s_b>0$. & \cref{sec:mx-methods} \\
$\mxrefscale_b$ & Prequantization reference scale $\max_{i\in\mxindexset_b}|y_i|/\mxrange$. & \cref{sec:mx-background} \\
$\mxrange$ & Positive element-range constant used by the reference scale rule. & \cref{sec:mx-background} \\
$\mxscalegrid,\ \mxelementgrid$ & Representable scale and element sets, respectively. & \cref{sec:mx-background} \\
$Q_\alpha,\ Q_E$ & Scale and element quantizers; $Q_E$ acts elementwise. Zero scale reconstructs to zero without division. & \cref{sec:mx-background} \\
$\mxmaxexponent$ & Maximum exponent of the element format in the power-of-two scale example. & \cref{sec:mx-background} \\
$K$ & Historical nominal scale-candidate slots, $K\in\{2,3,5,9\}$; clipping and stable deduplication leave at most $K$ unique candidates. & \cref{app:hash-search-experiment-details} \\
$\mxscale$ & Reference MX scale-selection function applied to a Gaussian block. & \cref{sec:mx-gaussian} \\
$i,\ b\dmx+i-1$ & Local coordinate $1\le i\le\dmx$ and its global index in block $b$; $(\y_b)_i=y_{b\dmx+i-1}$. & \cref{sec:mx-methods} \\
$\mxguidescale_b,\ \mxoutscale_b$ & Experiment initial guide scale and final represented output scale; equal for fixed-scale search. Reconstruction uses $\widehat{\y}_b=\mxoutscale_b\widehat{\x}_b$. & \cref{app:hash-search-experiment-details} \\
\addlinespace[5pt]
\multicolumn{3}{@{}l}{\textbf{Trellis and beam search}}\\*
$L,\ k,\ V$ & State-bit length, coded bits per scalar, and scalars per emission. $V\mid T$; $kV\in\mathbb Z$, $1\le kV\le L$. & \cref{sec:qtip-background} \\
$n,\ t$ & Number of trellis steps $n=T/V$ and step index $1\le t\le n$. & \cref{sec:qtip-background} \\
$\mathcal U$ & State set $\{0,\ldots,2^L-1\}$. & \cref{sec:qtip-background} \\
$u,\ v,\ u_{\mathrm{init}}$ & Predecessor, successor, and fixed initial state, all in $\mathcal U$. & \cref{sec:qtip-background,sec:beam_search} \\
$u_{1:n}$ & Admissible state sequence along the trellis path. & \cref{sec:qtip-background} \\
$C(u)$ & Reconstruction map $C:\mathcal U\to\mathbb R^V$. & \cref{sec:qtip-background} \\
$\trellissource_t,\ \trellisrecon_t$ & Source and reconstructed vectors in $\mathbb R^V$. & \cref{sec:qtip-background,alg:trellis_direct_decoding} \\
$\mathcal A$ & Directed edges defined by the bitshift transition. & \cref{eq:bitshift_trellis_transition} \\
$\operatorname{succ}(u)$ & Legal successor states of $u$, obtained by appending $kV$ bits. & \cref{eq:bitshift_trellis_transition} \\
$c,\ c_t$ & Branch label in $\{0,\ldots,2^{kV}-1\}$; stored $c_t=u_t\bmod 2^{kV}$ occupies $kV$ bits. & \cref{eq:bitshift_trellis_transition,sec:beam_search} \\
$d$ & Outdegree $d=2^{kV}$; distinct from target dimension $d=T$ and MX block size $\dmx$. & \cref{sec:qtip-background} \\
$B,\ \beamset_t$ & Integer beam width $B\geq1$ and indexed collection of at most $B$ retained path hypotheses. & \cref{sec:beam_search} \\
$\ell_t(u)$ & Local squared distortion $\|C(u)-\trellissource_t\|_2^2$. & \cref{eq:trellis-local-distortion} \\
$D(u_{1:n})$ & Total path distortion $\sum_{t=1}^n\ell_t(u_t)$; not the scale-cell probability. & \cref{eq:trellis-local-distortion} \\
$\beamhyp,\ \beamterminal_t(\beamhyp)$ & Hypothesis index and its terminal state in $\mathcal U$; different hypotheses can share a terminal state. & \cref{sec:beam_search} \\
$\beamcost_t(\beamhyp),\ \widetilde{\beamcost}_t(\beamhyp,v)$ & Retained path cost and expanded cost $\beamcost_{t-1}(\beamhyp)+\ell_t(v)$. & \cref{eq:beam_expansion} \\
$\beambackpointer_t(\beamhyp')$ & Predecessor-hypothesis index of retained hypothesis $\beamhyp'$; used for encoder traceback. & \cref{eq:beam-backpointer} \\
$\beamcandidates_t$ & Ordered expanded-candidate list before top-$B$ selection. & \cref{alg:trellis_beam_encoding} \\
$\graphG$ & Directed trellis graph $(\mathcal U,\mathcal A)$ of states and allowed transitions. & \cref{alg:trellis_beam_encoding} \\
\addlinespace[5pt]
\multicolumn{3}{@{}l}{\textbf{Conditional Gaussian guide}}\\*
$\randomvec Y,\ \randomvec X$ & Gaussian block $\randomvec Y\sim\mathcal N(0,I_{\dmx})$ and normalized block $\randomvec X=\randomvec Y/\mxscale(\randomvec Y)$. & \cref{sec:mx-gaussian} \\
$i,\ M$ & Coordinate index $i\in\{1,\ldots,\dmx\}$ and maximum magnitude $M=\max_i|Y_i|$. & \cref{sec:mx-gaussian-cdf-hash} \\
$s$ & Positive represented scale attained by $\mxscale$; conditioning fixes $\mxscale(\randomvec Y)=s$. & \cref{sec:mx-gaussian-cdf-hash} \\
$a(s),\ b(s)$ & Lower and upper maximum bounds in the scale preimage: $\{\mxscale(\randomvec Y)=s\}=\{a(s)\le M<b(s)\}$, with $0\le a(s)<b(s)<\infty$. & \cref{sec:mx-gaussian-cdf-hash} \\
$\tau,\ \stderf,\ \stdierf$ & Scalar magnitude argument, standard error function, and its inverse; the half-normal CDF is $\stderf(\tau/\sqrt2)$ for $\tau\ge0$. & \cref{sec:mx-gaussian-cdf-hash} \\
$\mxcellmass(s;d)$ & Endpoint-power difference $\stderf\!\left(b(s)/\sqrt2\right)^d-\stderf\!\left(a(s)/\sqrt2\right)^d$ for positive integer $d$; $\mxcellmass(s;\dmx)>0$ is the scale-cell probability. & \cref{sec:mx-gaussian-cdf-hash} \\
$F(\tau;s)$ & Conditional magnitude CDF $\Pr(|X_i|\le\tau\mid\mxscale(\randomvec Y)=s)$. & \cref{sec:mx-gaussian-cdf-hash} \\
$p,\ F^{-1}(p;s)$ & Interior probability $0<p<1$ and inverse conditional magnitude CDF. & \cref{eq:mx-gaussian-conditional-inverse} \\
$\tau^\star(s),\ p^\star(s)$ & Branch location $a(s)/s$ and corresponding CDF probability. $p^\star$ is defined in the main guide; $\tau^\star$ in its proof. & \cref{sec:mx-gaussian-cdf-hash,app:mx-gaussian-proof} \\
$Z_j,\ q$ & Proof-local magnitude $Z_j=|Y_j|$ and threshold $q=s\tau$. & \cref{app:mx-gaussian-proof} \\
$c$ & Proof-local nonnegative maximum bound in $\Pr(Z_i\le q,M<c)$; distinct from a trellis branch label. & \cref{eq:mx-gaussian-proof-rectangle} \\
\addlinespace[5pt]
\multicolumn{3}{@{}l}{\textbf{Integer hash and FP-Hash}}\\*
$\hashparams,\ \hashparams_\ell,\ \ell$ & Parameter family and output coordinate tuple; output coordinate index $1\le\ell\le V$. & \cref{eq:mx-hash-parameters} \\
$A_\ell,\ C_\ell$ & Unsigned 32-bit LCG multiplier and addend; $C_\ell$ is distinct from reconstruction map $C$. & \cref{eq:mx-hash-parameters} \\
$r_{\ell,j},\ m_{\ell,j}$ & Shifts $r_{\ell,j}\in\{1,\ldots,31\}$ ($j=1,2,3$); odd unsigned 32-bit multipliers ($j=1,2$). & \cref{eq:mx-hash-parameters} \\
$\lcg,\ \mxmix$ & LCG and XOR--multiply mixer for each output coordinate; integer products reduced modulo $2^{32}$. & \cref{eq:mx-hash-lcg,eq:mx-hash-mixer} \\
$w,\ \mxmixstep,\ \mxxorshift$ & Unsigned 32-bit mixer input; XOR--shift--multiply step and final XOR--shift function. & \cref{eq:mx-hash-mixer} \\
$\oplus,\ \gg$ & Bitwise XOR and logical right shift. & \cref{eq:mx-hash-mixer} \\
$w_\ell$ & Mixed 32-bit word for output coordinate $\ell$; hash state satisfies $L\le32$. & \cref{eq:mx-hash-mixer} \\
$\mxsignbit_\ell,\ U_\ell$ & Sign bit in $\{0,1\}$ and magnitude rank in $\{0,\ldots,2^{31}-1\}$; $U_\ell$ is distinct from set $\mathcal U$. & \cref{eq:mx-hash-sign-rank} \\
$p_\ell$ & Midpoint probability $(U_\ell+1/2)/2^{31}\in(0,1)$. & \cref{eq:mx-hash-interior-probability} \\
$h_{\hashparams,\ell},\ \mxhashvec$ & Quantized output coordinate emission in $\mxelementgrid$ and vector emission in $\mxelementgrid^V$. & \cref{eq:mx-hash-cdf-mapping} \\
$\randomvec S$ & Heuristic normalized Gaussian block $\randomvec S=\randomvec Y/\heuristicscale$. & \cref{sec:heuristic-fp-hash} \\
$\heuristicscale$ & Represented absmax reference scale in the heuristic. & \cref{sec:heuristic-fp-hash} \\
$\fpclipfactor$ & Heuristic clipping factor $1/\sqrt{2\ln(\dmx/\pi)}$. & \cref{sec:heuristic-fp-hash} \\
$\texttt{hash}_{\mathrm{qtip}},\ \texttt{hash}_{\mathrm{clip}}$ & Approximately Gaussian QTIP emission and its scaled, clipped, element-quantized heuristic adaptation. & \cref{sec:heuristic-fp-hash} \\
\addlinespace[5pt]
\multicolumn{3}{@{}l}{\textbf{Inverse-CDF lookup table}}\\*
$\lutslopes_0(s),\ \lutslopes_1(s)$ & Scale-dependent lower- and upper-branch affine slopes; the LUT superscript distinguishes them from trellis branch labels. & \cref{eq:lut-coefficients} \\
$\lutoffset(s)$ & Upper-branch affine offset; distinct from trellis outdegree $d$. & \cref{eq:lut-coefficients} \\
$\lutargument_\ell$ & Affine-transformed output coordinate probability passed to the shared inverse table. & \cref{app:efficient-lut} \\
$j,\ \lutknots_j,\ \lutvalues_j$ & Knot index $0\le j\le255$, increasing probability knots, and stored inverse values $\lutvalues_j=\stdierf(\lutknots_j)$. Interpolation intervals use $0\le j\le254$. & \cref{eq:lut-interpolation} \\
$\lutfunction$ & Piecewise-linear table approximation of $\stdierf$ on the covered probability domain. & \cref{eq:lut-interpolation} \\
$\widehat h_{\hashparams,\ell}$ & Quantized signed output coordinate emission using the inverse-CDF table approximation. & \cref{eq:lut-interpolation} \\
$\epsilon$ & Bound on $\stdierf$ approximation error on a covered interval; normalized pre-rounding contribution is at most $\sqrt2\epsilon/s$, excluding arithmetic error. & \cref{app:efficient-lut} \\
\end{longtable}
\endgroup


==> section_files/temp_results.tex <==
\clearpage
\section{temp results}
\suppressfloats[t]

\begin{table}[!h]
\caption{B-QMX: beam search in floating point followed by MX quantization. N-B-QFP: normalization using the MX scale, followed by beam search and final FP quantization. N-FPBS: normalization using the MX scale, with FP quantization applied inside the beam search.}
\label{tab:my-table}
\begin{tabular}{|l|cc|cc|}
\hline
Element Format & \multicolumn{2}{c|}{FP4}                 & \multicolumn{2}{c|}{FP8}                 \\ \hline
Hash Type      & \multicolumn{1}{c|}{1MAD}     & 3INST    & \multicolumn{1}{c|}{1MAD}     & 3INST    \\ \hline
B-QMX          & \multicolumn{1}{c|}{0.081712} & 0.080724 & \multicolumn{1}{c|}{0.070239} & 0.069162 \\ \hline
N-B-QFP        & \multicolumn{1}{c|}{0.086911} & 0.086334 & \multicolumn{1}{c|}{0.076241} & 0.074440 \\ \hline
N-FPBS         & \multicolumn{1}{c|}{0.075818} & 0.074079 & \multicolumn{1}{c|}{0.075692} & 0.073920 \\ \hline
Orcale         & \multicolumn{1}{c|}{0.069594} & 0.068359 & \multicolumn{1}{c|}{0.069594} & 0.068359 \\ \hline
\end{tabular}
\end{table}

